Heuristics for Quantum Compiling with a Continuous Gate Set

We present an algorithm for compiling arbitrary unitaries into a sequence of gates native to a quantum processor. As accurate CNOT gates are hard for the foreseeable Noisy- Intermediate-Scale Quantum devices era, our A* inspired algorithm attempts to minimize their count, while accounting for connectivity. We discuss the search strategy together with metrics to expand the solution frontier. For a workload of circuits with complexity appropriate for the NISQ era, we produce solutions well within the best upper bounds published in literature and match or exceed hand tuned implementations, as well as other existing synthesis alternatives. In particular, when comparing against state-of-the-art available synthesis packages we show 2.4x average (up to 5.3x) reduction in CNOT count. We also show how to re-target the algorithm for a different chip topology and native gate set, while obtaining similar quality results. We believe that empirical tools like ours can facilitate algorithmic exploration, gate set discovery for quantum processor designers, as well as providing useful optimization blocks within the quantum compilation tool-chain.

==> abstract.tex <==



==> misc.tex <==
\subsection{To Do}

\begin{enumerate}
\item Mention Shende synthesis paper - topology adds a factor of nine in CNOTs ...


\item Raban and Shende - algorithms only, upper bounds with no implementation


\item Sutton - not that many real algorithms to compute CSD

\item CSD may not apply to qutrits ...

\item ~\citep{MIM13} Clifford+T - they do Toffoli, 10 CNOTS + 2 Ts, don't scale...

\item\citep{ionsynth} - needs discussion. Numerical optimization with
  predecomposed matrix with MS gates (equivalent to CNOTs). 3 qubits
  in 8 gates - we do better. Not topology aware, does not matter for
  MS. Decomposition fixed for qubits and CNOTs - can't specialize
  easily. Search strategy - random seed and search ..

  \item \citep{qaqc} - same idea for numerical optimization, but use
    quantum computer for it. Show results for 2 qubits, which we
    match. Simulated annealing over all sequences of length L. Same
    metric based on Hilbert-Schmidt.
  
\item Discussion section - what is synthesis good for. We show its a
  good tool for small circuits, probably gate discovery, circuit
  optimization with partitioning...
  Discuss scalability trends and possible approaches: partitioning,
  norm selection ...

\end{enumerate}

==> paper/abstract.tex <==
\begin{abstract}
 {\it We present an algorithm for compiling arbitrary unitaries into a
 sequence of  gates native to a quantum processor. As accurate \cn gates are
 hard for the foreseeable
 Noisy-Intermediate-Scale Quantum devices era, our  A* inspired algorithm
 attempts  to minimize their count, while prioritizing connectivity. We discuss the search strategy
 together with ``metrics'' to expand the solution frontier. We
 demonstrate multiple uses:  1) compiling unitaries to circuits; 2)
 gate set exploration; and 3) circuit optimization. Although we cannot provide hard
 optimality guarantees, in each case we produce solutions well within the best lower
 bounds published in literature and match or exceed hand tuned
 implementations. We also show how to re-target the algorithm for a different
 chip topology and native gate set, while obtaining similar quality
 results. We believe that empirical tools like ours can
 facilitate algorithmic exploration, gate set discovery for quantum processor designers,
as well as providing useful optimization blocks within the quantum compilation tool-chain.}
\end{abstract}


==> paper/algo.tex <==
\section{Synthesis Algorithm}
\label{sec:alg}

Our goal is to design an algorithm that addresses current perceived
shortcomings of synthesis  
and that  can be  easily extended to new hardware in order  to enable design space exploration in
quantum programming. To be useful during the NISQ device era we use circuit depth
as primary optimality criteria, while allowing for specialization to a
particular chip
topology.  We target directly the native gate set
associated with a particular processor and attempt to minimize the \cn
count in the generated circuit. The synthesis algorithm described in the rest of this section uses a
greedy search strategy, inspired by the A*
algorithm~\citep{astar}. 

Before dwelling into synthesis  details, we
provide the intuition behind A* searches. The A*
algorithm has been developed for graph traversals and it attempts to
find a path between a start and target node. It uses a greedy
approach where at each step  partial solutions are
extended based an a cost function. The algorithm maintains a tree of
paths from the start node, and the solution
is the path with the smallest cost.  Given a partial solution, the algorithm extends it
based on the cost of its already computed path and an estimate of the
cost required to extend it all the way to the target. Assuming that $n$
is the next node,  A* selects the path that minimizes
$f(n) = g(n) + h(n)$  where
\begin{itemize}
\item $f(n)$ is the cost of the path through node $n$
\item $g(n)$ is the cost of the path from the start to $n$
  \item $h(n)$
is a heuristic function that estimates the cost of the cheapest path
from $n$ to the target
\end{itemize}
The algorithm terminates when it reaches the target node or if there
are no paths eligible to be extended. The heuristic function is
problem-specific and directly determines the time complexity of A*. If the heuristic function is {\it admissible},
meaning that it never overestimates the actual cost to get to the target, A* is guaranteed to return a least-cost path. 



\newcommand{\us}{U_{start} }
\newcommand{\uss}{$U_{start}$ }
\newcommand{\ug}{U_{goal} }
\newcommand{\ugs}{$U_{goal}$}
Informally, we cast our synthesis algorithm into an A* inspired
framework as follows. Given the unitary \uss associated with a
particular algorithm, we want to determine the unitary \ugs , where
$D(\us,\ug) \le \epsilon$. Here $D(U_1,U_2)$ is the distance
function that indicates how well $U_2$ approximates $U_1$ and
$\epsilon$ is an acceptability criteria used to terminate
the search for \ugs. That is, the search will terminate upon finding
the first acceptable \ugs. 


The evolution of the search on a three qubit example is depicted in
Figure~\ref{fig:usearch}. Let \ugs \ be the unitary associated with the
transformation we compile. This is a matrix where all entries are
floating point numbers.  The initial solution approximation is
$U_{goal}^0$, obtained by placing arbitrary SU(2) unitaries on each
qubit. These unitaries are represented in their most generic
continuous (or variational) parameterized form
$U3(\theta,\phi,\lambda)$ introduced in Equation~\ref{eq:u3}, where
each gate is fully specified using three independent parameters $(\theta,\phi,\lambda)$.

For convenience in Figure~\ref{fig:usearch} we use the following
notations. For the parameterized unitary $U3(\theta,\phi,\lambda)$ we
use the shorthand notation U. We also annotate the unitaries with the 
qubit they apply on and with their  application in time. For example
$U_0^1$, denotes applying the unitary $U3(\theta,\phi,\lambda)$ to
qubit zero at time step one. Similarly, $U_0^2$ denotes the next
unitary applied to qubit zero after time step one. Without the
shorthand notation, to fully characterize the circuit we would need six
parameters as we apply in sequence 
$U3_0^1(\theta_0^1,\phi_0^1,\lambda_0^1)$ and
$U3_0^2(\theta_0^2,\phi_0^2,\lambda_0^2)$ to qubit zero.

Let the current partial solution be denoted by $U_{goal}^{current}$. We maintain two
representations for $U_{goal}^{current}$, one parameterized by the already
placed gates/unitaries and another one where gates are numerically
instantiated.

At each step, the instantiation of $U_{goal}^{current}$ is performed by
a numerical 
optimizer that minimizes $D(U_{start}-U_{goal}^{current})$. This amounts to
computing values for all the parameters
$\theta_i^j,\phi_i^j,\lambda_i^j$ throughout the circuit. 

At each step, the algorithm tries to expand the existing solution
using the building block described in Figure~\ref{fig:usearch}(A).  It
will consider all solutions where it places the block on a pair of
qubits that are physically connected. Thus we consider a number of
independent partial solutions equal to the number of links in the chip
and in the
expansion step we add six more independent parameters. For
a circuit with $N$ qubits, this building block amounts to placing a
\cn gate on two qubits, followed by generic SU(2) operations on the
same qubits. The $N-2$ unaffected qubits are assigned the identity operations
denoted by $I_2$. As described the unitary associated with this block
is $U_{expansion} =  (I_2 \otimes ... \otimes I_2 \otimes
U(\theta_1,\phi_1,\lambda_1) \otimes U(\theta_2,\phi_2,\lambda_2))(I_2
\otimes  ... \otimes I_2 \otimes CNOT)$, where   $I_2$is the identity
$2 \times 2$ matrix and $CNOT$ is the CNOT unitary.  For each of the
possible next solutions we perform again the distance minimization,
which amounts to $U_{goal}^{current} = minimize[ D(U_{start} -
U_{expansion}U_{goal}^{current})]$.


The search stops when it finds an instantiation whose distance is
smaller than a given error threshold or when exceeding an upper bound
on acceptable circuit \cn depth. 


\begin{figure*}
  \begin{tabular}{c}
\begin{minipage}{\textwidth}
  \centerline{\includegraphics[width=3in,height=1in,keepaspectratio]{expansion}}
  \centerline{(A)}
\end{minipage} \\

    \begin{minipage}{\textwidth}
  \includegraphics[width=5in,height=3in]{usearch}
 \centerline{ (B)}
  \caption{\label{fig:usearch} \it  (A) Basic circuit block used for
    expanding the solution. We generate all alternatives where this
    structure is placed on linked qubit pairs. Each step adds six
    additional parameters to the optimization problem.  (B) Example evolution
    of the search algorithm for a three qubit circuit. We start by placing a layer of single
    qubit gates, then generate the next two possible solutions. Each
    is evaluated and in this case the upper circuit is closer to the
    target unitary. This circuit is then expanded with its possible
    two successors. These are again instantiated by the optimizer. The
    second circuit from the top has an acceptable distance and is
    reported as the solution. The path in red  shows the evolution of
    the solution. The solutions enclosed by the dotted line have been
    evaluated during the search.}
 \end{minipage} \\

 \begin{minipage}{\textwidth}
  {\tiny \inputpython{pseudocodev2.txt}{0}{100}}
 \caption{\label{fig:alg} \it Pseudocode for A* inspired search
   algorithm. }
\end{minipage} \\
\end{tabular}
\end{figure*}

==> paper/analysis.tex <==
\section{Algorithm Properties}
\label{sec:prop}

The algorithm performance is determined by the complexity of the
$A^*$ search combined with the growth of the parameter optimization
space with circuit depth.

The time complexity  depends on the heuristic. In the worst
case, the number of nodes expanded is proportional to number of qubit
links and circuit depth $O(L^d)$, where $L$ can be thought as the
average number of links explored per intermediate solution. Given the
availability of solution existence theorems as described in the related
work Section~\ref{sec:related}, the algorithm will terminate.


Figure~\ref{fig:evol} shows the evolution of a search correlating
circuit depth to solution distance for the QFT three
qubit circuit. At each depth two alternatives (two links
between qubits) are evaluated and the algorithm does not
backtrack. This is an example of a very efficient search. At the
time of this submission, we are still analyzing data from all 
 runs, and plan to provide the empirical analysis for the
final version. For algorithms such as Fredkin the algorithm
backtracks. 

Note that our implementation explores the parallelism available during
the search and evaluates concurrently all next solutions; this
amount to evaluating a number of tasks equal to the number of physical
connections in the chip. At the
time of this writing we rely on the Python {\tt multiprocessing.pool}
infrastructure for resource management. We believe
we can easily speed up the search with a more coordinated parallel
implementation as discussed in Section~\ref{sec:related}.

If the heuristic function used to expand a partial solution is
admissible, meaning that it never overestimates the cost of reaching
the goal, $A^*$ is optimal. If the heuristic function is monotonic,
partial solutions with a cost greater than the recorded minimum need
not be considered during expansion.  In our case, the distance
function is not monotonic and we do may end up considering all partial
solutions. The lack of monotonicity is 
illustrated in Figure~\ref{fig:evol}.


\begin{figure}
 \comment{ [width=3in,height=1in]}
 \includegraphics[width=3in,height=1.5in,keepaspectratio]{deptherror}
 %\vspace{-.3in}
 \includegraphics[width=3in,height=1.5in,keepaspectratio]{params}
  \caption{\label{fig:evol} \it (Left) Evolution of circuit depth and
    distance to solution during synthesis of \red{\bf WHAT?} on a
    \red{\bf how many} qubit circuit. The solution has a depth of 9
    CNOT gates. We also plot the evolution of the distance through the
  search. As seen at steps 10 and 11, distance function is not monotonical.}
 \end{figure}


Besides algorithmic complexity, optimizer scalability with parameters is another
factor that determines performance. In fact, this is the currently
limiting factor. The algorithm starts by adding an
initial layer of single qubit gates, each with three free
parameters. At each expansion step, we add the building block
described in Figure~\ref{fig:alg}, with additional six free
parameters. Thus, for a circuit with depth $d$, the total number of
parameters is $Num\_Params = 3*Q + 6*d$.  Table~\ref{tab:params}
shows the upper bounds on parameter count, when considering the
theoretical upper bounds on circuit depth presented by~\citet{raban}. 

\begin{table}[h]
\centering
{\small
\begin{tabular}{l|l|l|l|l|l}
n\\ m       & 0 & 1& 2&3&4 \\ \hline
2      & 12& 18&{\bf 24}&-&- \\
3      & 27&63& 93&{\bf 129}& -  \\
  4     & 60 &144&54&336&{\bf 612}  \\

\end{tabular}
}
\caption{\label{tab:params} \it Upper bound on parameter count when
  synthesizing a $m$ qubit circuit into  $n$ qubits, with $m \le
  n$. The bounds are from~\citet{raban}. Note that while the CNOT
  counts grow very fast, the empirical approach may derive much
  shorter circuits. For example, for all three qubit circuits tested, we
obtain depths of nine, which amounts to 63 parameters instead of 129. }

\vspace{-.2in}
\end{table}







\subsection{Numerical Optimizers for Circuit Synthesis}

A closer look at the interaction between numerical optimization and
circuit synthesis is required in order to develop robust and scalable
quantum circuit synthesis.

Numerical optimization has a long and distinguished~\citep{Rios2013}
research track record. Their design and performance is determined by
the mathematical properties of the objective function. Tuning and
choosing the right optimizer for a particular domain is still very
much of a black-art.

The most
scalable and efficient methods are developed for objective functions
that allow a gradient or derivative computation. Under the assumption that the objective function is continuously
differentiable, quasi-Newton methods can be used. These approximate
the first (and sometimes second) derivatives by evaluations along an
estimated gradient. From these the Broyden-Fletcher-Goldfarb-Shanno
algorithm (BFGS) is deemed as scalable with parameters and widely
used in practice. Previous work in circuit synthesis~\citep{ionsynth}
with numerical optimization uses it directly.



From the beginning, our intuition was that the objective function
during synthesis may not allow gradients or derivatives and we need to
examine derivative-free methods which employ sampling (``blackbox
optimization'') and do not impose any requirements on the objective
function. 
Our choice was the Covariance Matrix Adaptation Evolution
Strategy~\citep{cmaes}, which is a genetic algorithm implemented in
multiple languages including C, Matlab, and Python. We have chosen it
based on the availability of a Python implementation.  Mutation is
performed by a perturbation with expected value zero and a covariance
matrix which is iteratively updated to guide the search towards areas
with expected lower objective values. CMA-ES is expected to scale up
to hundreds of parameters. On the other hand, when compared to other
methods~\citep{Rios2013} it may perform a large number of function
evaluations during search, which slows it down.

For our purposes, CMA-ES was able to successfully handle circuits with
a small number of qubits. Due to its genetic approach,
the algorithm exhibits randomness and non-deterministic behavior, and
in order to obtain the lowest depth circuit there were cases where we
had to synthesize repeatedly. Fortunately, the number of trials
required was low (two)  and the differences in depth were always one level
(e.g.  four versus five CNOT  gates). 


Some synthesis runs were slow, in particular for the Fredkin gate
where the search backtracks after exploring long paths (limited to 20
depth for three qubits). These motivated us to examine other
optimizers. We have started with BFGS, which did not work at all for
this circuit as it gets stuck at local minima.  This is contrary to
the experiences reported in~\citep{ionsynth}. Perhaps the difference
is explained by the fact that~\citet{ionsynth} examine only randomly
generated unitaries, rather than well defined algorithms or gates. 


Overall, we found limited availability of open source derivative-free optimizers
implemented in anything else but MATLAB.

\subsection{Reducing the Number of Free Parameters}

Besides choosing better optimizers, another strategy is to try to
reduce the number of parameters evaluated during the search.  Our idea
was to identify a circuit prefix that is kept constant during the
search and re-synthesize only a frontier of parameters. In the terms
from Figure~\ref{fig:usearch}, in the simplest
case  we considered  keeping the partial solution 
$U_{goal}^i$ at step $i$ constant across two expansion steps and synthesizing
values only for $U_{goal}^i(ct) \otimes U_{expansion}^i \otimes
U_{expansion}^{i+1}$. As the distance function is not monotonic, this
strategy slows down the search due to excessive backtracking.

Another empirical approach that we have considered is to examine the
numerical values of the parameters during the search and see if we can
determine circuit regions that are somewhat
constant. Figure~\ref{fig:evol}(right) shows the evolution of the
parameters associated with the first level of single qubit gates. This
irregular behavior occurs at all levels.

For brevity, we will not describe all attempts but mention that all
resulted in excessive backtracking and overall slowdown.

\subsection{Greedy Search, Topology  and Degrees of Liberty}


The results in Table~\ref{tab:res} illustrate quantitatively the
challenges faced by heuristic approaches. There is a degree of
randomness in our approach introduced by the CMA-ES
optimizer. Furthermore, the search strategy is greedy and not
guaranteed to find the optimal result.

The combination of these factors is apparent. First, there are cases (Fredkin) where we need  two synthesis runs in
order to match the best known solution. Furthermore, there are cases
where when moving from line to bowtie topology  the algorithm
finds a longer depth. This  happens for HHL and CNOT gates, or QFT and
Toffoli for $\sqrt{\cn}$ gates.  In general, the more degrees of
liberty associated with the problem (links or parameters), the higher
the chance the search finds an acceptable but suboptimal solution.
As we have evidence that more constrained searches found better
solutions, one venue is to empirically tune the algorithm with a
tighter acceptance $\epsilon$ criteria in these cases. We plan to  perform
this for the final version of the paper. 

==> paper/background.tex <==
\section{Background }
\label{sec:bg}

In quantum computing, a qubit is the basic unit of quantum information. Physically, qubits are two-level quantum-mechanical systems, whose general
quantum state is represented by a linear combination of two orthonormal basis states (basis vectors).  The most common basis is the equivalent
of the 0 and 1 values used for bits in classical information theory, \\
respectively $\ket{0} = \begin{bmatrix} 1 \\ 0 \end{bmatrix}$ and
$\ket{1}$ = $\begin{bmatrix} 0 \\ 1 \end{bmatrix}$. The generic qubit state is a superposition of the basis states, i.e. $\ket{\psi} = \alpha \ket{0} + \beta \ket{1}$, with $\alpha$ and $\beta$ complex amplitudes such as $|\alpha|^2+|\beta|^2=1$.

Although it appears there are four degrees of freedom in the generic qubit state $\ket{\psi}$, the normalization constraint removes one degree of freedom. Thus qubits can be represented in Hopf coordinates~\citep{Hopf1931} with three degrees of freedom $\alpha = e^{i\psi}cos\frac{\theta}{2}$ and $\beta = e^{i(\psi+\phi)}sin\frac{\theta}{2}$. Furthermore, since the phase of the $e^{i\psi}$ has no physical observability, the notation can be further simplified to two degrees of freedom, with $\phi$ the significant relative phase: $\alpha = cos\frac{\theta}{2}$ and $\beta = e^{i\phi}sin\frac{\theta}{2}$. This is usually visualized using the Bloch sphere.


\subsubsection{Gate Sets in Quantum Computing} The prevalent model of quantum computation is the circuit model introduced by~\citet{qcircuit}, where information carried by qubits  (wires) is modified by quantum gates, which mathematically correspond to unitary operations. A complex square matrix U is {\bf unitary} if its conjugate transpose $U^*$ is also its inverse, i.e. $UU^* = U^*U = I$.


In the circuit model, a single qubit gate is represented by a $2 \times 2$ unitary matrix U. The effect of the gate on the qubit state is obtained by
multiplying the U matrix with the vector representing the quantum state $\ket{\psi'} = U\ket{\psi}$.
 

The most general form of the unitary associated with a single qubit
gate is \begin{equation} \label{eq:u3} \begin{pmatrix} cos{\frac{\theta}{2}}  &
  -e^{i\lambda}sin{\frac{\theta}{2}} \\
  e^{i\phi}sin{\frac{\theta}{2}} &
  e^{i\lambda+i\phi}cos{\frac{\theta}{2}}\end{pmatrix}\end{equation} This is
sometimes referred to as $U3(\theta,\phi,\lambda)$, a ``continuous''
gate representation or  a ``variational'' gate representation.


In quantum computing theory, a set of quantum gates is {\it universal} if any computation (unitary transformation) can be approximated on any number of qubits to any precision when using only gates from the set. On the hardware side, quantum processors expose a set of native gates which constitute an universal set.  Quantum processors built from superconducting qubits usually provide a gate set consisting of single qubit rotations ($R_x$, and $R_z$) and two qubit \cn gates.  The unitaries for these gates are
\begin{equation} \label{eq:rs}
R_x(\theta) =  \begin{pmatrix} cos{\frac{\theta}{2}}  & -i sin{\frac{\theta}{2}} \\  -i sin{\frac{\theta}{2}} & cos{\frac{\theta}{2}} \end{pmatrix}, R_y(\theta)= \begin{pmatrix} cos{\frac{\theta}{2}}  & -sin{\frac{\theta}{2}} \\   sin{\frac{\theta}{2}} & cos{\frac{\theta}{2}} \end{pmatrix},  R_z(\phi)= \begin{pmatrix} e^{-i{\frac{\phi}{2}}}  & 0\\   0 &  e^{i{\frac{\phi}{2}}}\end{pmatrix}
\end{equation}


A \cn, or controlled NOT gate, flips the target qubit {\it iff} the control qubit is $\ket{1}$ and it has the following unitary \begin{equation} \label{eq:cn} CNOT = \begin{pmatrix}  1 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 \\ 0 & 0 &0 & 1 \\ 0 & 0 & 1 & 0 \end{pmatrix}\end{equation}



\subsubsection{Quantum Circuits} Any quantum computation (referred to also as transformation or algorithm) is represented by a unitary matrix. When running on hardware, this unitary is ``instantiated'' into a set of terms whose product is ``equal'' to the target unitary. The terms are selected from the hardware native gate set and this instantiation represents the circuit that will implement and compute the original algorithm. Thus, a circuit is described by an  evolution in space (application on qubits) and time of gates.   Figure~\ref{fig:circ} shows an example circuit that applies single qubit and \cn gates on three qubits.



\subsection{Background on Quantum Circuit Synthesis}
\label{sec:bg}
A quantum transformation on $n$ qubits is represented by a unitary matrix U of size $2^n \times 2^n$. The goal of quantum circuit synthesis is to decompose U into a product of terms, where each individual term captures the application of a quantum gate on individual qubits.  This is depicted in Figure~\ref{fig:circ}.

The quality of a synthesis algorithm is evaluated by the circuit depth it produces (number of terms) and by how well the solution approximates the original matrix. Exact synthesis computes a solution that is numerically equal to the original matrix.  Approximate synthesis computes a solution that is acceptable but not numerically equal to the original matrix. This occurs when applying heuristics  to limit the circuit depth, or in the cases where an exact solution is not guaranteed. 

We discuss in more detail related work in synthesis in Section~\ref{sec:related} and summarize in this section only the pertinent state-of-the-art results for  NISQ devices.

Reasoning whether a synthesis algorithm is exact is subtle in particular on NISQ devices. For example,~\citet{ctmq} describe an algorithm for exact synthesis using Clifford + T gates. On current devices, T gates are not native and implemented as approximations, thus their algorithm ultimately may produce an approximation. \comment{In our work we target only gate sets native to a particular quantum processor implementation. }

The other metric of importance when evaluating synthesis algorithms is circuit depth, with the implicit assumption that shorter depth is optimal. As \cn gates are problematic on NISQ devices, state-of-the-art approaches~\citep{raban,synthcsd} directly attempt to minimize their count. \cn count is a direct indicator of overall circuit length, as the number of single qubit generic gates  introduced in the circuit is similar, to a constant given by decomposition rules. \comment{In our work we take a similar tack and attempt to minimize \cn count.}



When reasoning about single qubit unitary operations, the $ZYZ$ decomposition rule states that any unitary $U$ can be rewritten as $U=e^{i\alpha}R_x(\beta)R_y(\gamma)R_z(\delta)$, with a proof available in~\citet{Nielsen-2010}; thus synthesis can focus on minimizing \cn count.

There are two types of synthesis approaches that we use to drive our design goals. The more rigorous and theoretical approaches use linear algebra techniques such as Cosine-Sine Decomposition~\cite{raban,synthcsd} to prove upper bounds on circuit depth. Most do not seem to provide numerical implementations or results on actual circuits. We use the published upper bounds for the evaluation of our approach, as well as an internal stopping  criteria for the search algorithm. Empirical approaches use search heuristics for decomposition. From these, we are mostly interested in numerical optimization approaches~\cite{ionsynth,qaqc} which are similar in spirit to our proposed solution. These tend to generate shorter circuits, but implicitly assume full qubit connectivity. We compare against their results to estimate the efficacy of our technique.


{\it Table~\ref{tab:depth} presents the best known upper bounds on \cn count for synthesis algorithms.} We present only data for short circuits when synthesizing a unitary of size $m$ into $n > m$ qubits. Note that for three qubits the bound is 20 \cn, while for four qubits it is 100 \cn.  Asymptotically, the tightest bound is introduced by~\citet{raban} to a \cn count of $0.16*(4^m+2*4^n)$. Because of the exponentiation, for current generation devices it is important to demonstrate quantitatively that we can attain shorter depth.

Another important aspect when evaluating synthesis approaches is the {\it   ability to take chip qubit connectivity into account}. Topology agnostic approaches may place \cn gates between qubits that are not physically connected. In these cases, the backend compilers need to introduce $SWAP$ gates, each $SWAP$ gate being implemented using three \cn gates.

Early synthesis algorithms implicitly assumed full qubit connectivity, while more recent approaches provide bounds when specializing for topology. The algorithms presented by~\citet{synthcsd} increase the \cn count by a factor of nine when restricting topology to a nearest-neighbor interaction, while~\citet{raban} claim a factor of four.

Note that these are bounds derived when restricting topology from all-to-all to nearest-neighbor, and their generalization\footnote{Intuitively, the bound is likely to be lower for higher connectivity.}  to other topologies such as the IBM Q bow-tie it is not clear. Furthermore, even when these bounds for topology specialization are available, not enough quantitative data is available to judge the quality of a synthesis algorithm. The topology agnostic bounds seem to be loose and most, if not all, studies do not present data when compiling realistic circuits or algorithms. The little data that is available  is provided for random unitaries.

When specializing for topology the bounds are even looser. For a $m$ qubit unitary, existing algorithms can generate circuits with ancilla qubits resulting in $n > m$ qubit circuits.  Intuitively these should have a shorter length than the non-ancilla synthesis when topology is restricted, regardless of their theoretical higher bound.
We did not find much quantitative data for sample circuits in these cases, and there seem to be little guidelines for approaching the problem.  




\begin{figure}
 \comment{ [width=3in,height=1in]}
 \includegraphics[width=2in,height=.6in,keepaspectratio]{circ1}
 %\vspace{-.3in}
 \includegraphics[width=2in,height=.4in,keepaspectratio]{tensor}
  \caption{\label{fig:circ} \it Unitaries (left) and tensors products (right). The unitary U represents a $n=3$ qubit transformation, where  U is a $2^n \times 2^n$  ($8 \times 8$) matrix. The unitary is
    implemented (equivalent or approximated) by the circuit on the right hand side. The single qubit unitaries are $2 \times 2$ matrices, while CNOT is a
    $2^2 \times 2^2$ matrix. The computation performed by the circuit is $(U3 \otimes U4 \otimes U5)(I2 \otimes CNOT)(U1 \otimes U2 \otimes U3)$, where   I2 is the identity $2 \times 2$ matrix and $ \otimes $ is the tensor product operator. The right hand side shows the tensor product of $ 2 \times 2$ matrices. }
 \end{figure}


 \begin{table}[h]
\centering
{\small
\begin{tabular}{l|l|l|l|l|l}
n \ m       & 0 & 1& 2&3&4 \\ \hline
2      & 1& 2&{\bf 3}&-&- \\
3      & 3 &9& 14 &{\bf 20}& -  \\
  4     & 8 &22 &54&73 &{\bf 100}  \\

\end{tabular}
}
\caption{\label{tab:depth} \it Upper bound on CNOT gate count when synthesizing a $m$ qubit circuit into  $n$ qubits, with $m \le n$. Data is presented by ~\citet{raban}. The counts for $n=m$ are  introduced by ~\citet{synthcsd}. The counts for state preparation ($m = 0$) on two and three qubits are presented by ~\citet{znidaric}, and the count for state preparation on four qubits is introduced by~\citet{raban}. The generalization and upper bound of  is derived by~\citet{raban}. Note that the CNOT counts grow very fast. For example, the upper bound on any unitary on 10 qubits is about about 500,000 CNOT gates.}

\vspace{-.2in}
\end{table}




\subsubsection{Reasoning About Circuits and Algorithm Equivalence}

A quantum transformation can be implemented by multiple distinct quantum circuits, that is when reasoning in terms of unitaries, there exist multiple decompositions of the unitary into terms that represent gates. Furthermore, when running on hardware, the unitary executed is often subtly different from the intended unitary.

Thus, it is often the case where we want to perform a particular quantum operation $A$ and because of external constraints we end up performing an approximation $B$, where $B \ne A$.  Given two algorithms $A$ and $B$, we want to determine which was executed, as well as how ``close'' are they in computing the same transformation. This is often referred to as distinguishability in literature and  several metrics with operational motivation have been proposed.  Metrics such as trace distance and fidelity~\citep{gilchrist,breuer,Nielsen-2010} have been proposed for distinguishing states. Metrics such as the diamond norm~\citep{Kitaev:2002} have been introduced to distinguish processes (algorithms) and are better suited for ``static'' reasoning about circuits, without circuit dependence.

Synthesis algorithms use norms  to assess the solution quality, and their goal is to minimize $\norm{U - U_S}$, where $U$ is the unitary that describes the transformation and $U_S$ is the computed solution. Approximate synthesis algorithms choose an error threshold $\epsilon$ and use it for convergence criteria, $\norm{U-U_S} \le \epsilon$. When reasoning in terms of norm distance, smaller is always better. On the other hand, there is little or no quantitative data available to relate the error threshold $\epsilon$ to observable circuit behavior and error metrics on output/states. As the error threshold determines both
convergence ``speed'' and quality of solution, algorithm designers use heuristics to determine appropriate values, but this algorithmic tuning is still a black art.  Early synthesis algorithms use the diamond norm, while more recent efforts~\citep{qaqc,HSnormsynth} use the Hilbert-Schmidt  inner product between the conjugate transpose of $U$ and $U_s$. This is motivated by its lower computational overhead. We describe our choices  in Section~\ref{sec:impl}.
\begin{equation} \label{eq:hsn}
   \langle U, U_s \rangle_{HS} = \Trace(U^{\dag} U_s)
\end{equation}




\subsection{Quantum Processors}
\label{sec:qps}
We demonstrate synthesis results on two distinct architectures built using transmon~\citep{transmon} superconducting qubits. We initially  targeted the \qnl chip developed by the UC Berkeley
Quantum Nanoelectronics Laboratory ~\citep{qnl}, with eight
superconducting qubits connected in a line topology and with a native
gate set consisting of rotations and \cn gates \{$R_x(90),
  R_z(\theta), CNOT$\}. We then consider a chip with better connectivity, such as the ``bowtie'' employed in
  the IBM Q 5~\citep{ibmq5}, but a similar native gate set. Note that other superconducting qubit architectures support very similar  native gate sets, some with restricted topology~\citep{tqfrigetti}, others with richer connectivity~\citep{Google-2018}.  We believe that our results are easily generalized across superconducting qubit architectures which tend to support rotations and a single two qubit gate (\cn, CZ or SWAP).

 While topology is important for superconducting qubits, implementations using trapped ion~\citep{itq} qubits provide all-to-all connectivity through M\o lmer-S\o rensen~\citep{msg}  gates. Thus synthesis algorithms that target these architectures need not be topology aware. 
  
  

  

==> paper/conc.tex <==
\section{Conclusion}
\label{sec:conc}

In this work we have shown methods to compile arbitrary quantum
unitaries into a sequence of gates native to several superconducting
qubit based architectures. The algorithm we develop is topology aware
and it is easily re-targeted to new gates sets or topologies. We
evaluate behavior on several proper algorithms and randomized
unitaries. Results indicate that we can match the shortest depth
published circuit implementation. Our exploration of $\sqrt{\cn}$ and
qutrit 
gates is of direct interest to hardware and algorithm designers.  We
believe that targeting these gates is perhaps beyond the capabilities
of existing published techniques.  We also provide a performance
analysis of synthesis using numerical optimization. Due to our more
extensive benchmark set, we uncover limitations in available
optimizers and implicitly in previous approaches. Looking forward,
better numerical optimizers are required for enhancing the
palatability of quantum circuit synthesis. These will alleviate some of the
need for developing better search algorithms.

==> paper/disc.tex <==
\section{Discussion}
\label{sec:disc}

Overall, we believe our results are very encouraging and show the
general applicability of quantum circuit synthesis techniques during
the NISQ decade(s). We have shown concrete results where we match the
shortest known depth for several algorithms or two qubit gates, we
have shown applicability to gate discovery  and to circuit
optimization.

We attain extensibility  by a combination of design
choices.  First, we target directly the hardware native gate set. This is easily retargetable, as illustrated by the set of
experiments using $\sqrt{CNOT}$ gates.
Topology awareness is attained by using
directly the information about chip connectivity  when devising the
part of the search strategy that attempts to expand on the frontier of
partial solutions. This is also easily retargetable as illustrated by
the experiments on the line and bowtie topologies. 

Due to its potential,  we believe a roadmap for synthesis targeting
NISQ devices
is worth developing. Our study illustrates some of the solutions, as
well as the associated open problems. For practical purposes,
scalability is as important as quality of solution (short depth circuits). For the near
future, scalability at small qubit scale is worth exploring as it will
lead to establishing robust building blocks when considering
scalability with qubits.

\parah{Synthesis for early NISQ (small) circuits} This is the 
state-of-the-art and based on our preliminary experiences we believe
we can extend synthesis to handle systems up to sixteen
qubits. There are several orthogonal directions to pursue to improve speed:
\begin{itemize}
\item {\it Better parallelization of the search algorithm.} The current
  approaches do not offer any level of coordination between the
  parallel evaluations of solutions. One possible direction is to
  develop more coordinated algorithms for parallel searches.
  All existing search approaches assume the cost per step is
independent of depth in the solution tree. Another direction worth pursuing seems to be developing algorithms
  that guide the search using a heuristic that combines solution
  quality with expansion cost.   One idea is to develop hybrid techniques that combine
  breadth-first with depth-first traversals that account for the
  number of parameters, as inspired by~\citet{Beamer2012} in the graph
  algorithms realm.  
  
\item {\it Better numerical optimizers.} The judicious choice of the numerical optimizer is probably the most
important factor. ~\citet{Rios2013} provide a very useful overview of
derivative-free methods. Based on their recommendations, the first
step is to select the best known derivative-free methods such as
TOMLAB/MULTIMIN, TOMLAB/GLCCLUSTER, MCS or TOMLAB/LGO. The second
step is to employ meta-optimization techniques that combine different
approaches. For example, from all optimizers surveyed, TOMLAB/OQNLP, NEWUOA
and TOMLAB/MULTIMIN are reported to be best in terms of refining a
near-optimal solution. Moving from CMA-ES to TOMLAB/MULTIMIN or to a
solution where a partial solution from one optimizer is passed into
another seem as sensible approaches. We are also considering building
ad-hoc optimizers for synthesis based on tensor networks. These have
the advantage of high GPU performance. 

Note that  the choice is limited due
to lack of availability of open source Python or C based implementations.  
  \item Methods to bound the number of parameters.  In our opinion these are the most
    promising in terms of improving speed to solution. Our initial
    attempts to recognize and ``memoize'' blocks of parameters that
    are slowly changing during synthesis failed, but there are plenty
    of unexplored venues in this direction.  Another possible
    direction is to consider hybrid approaches that combine matrix
    decomposition methods such as Cosine-Sine with numerical
    optimization methods on subterms. This is one of our areas of
    future work.
 \end{itemize}

 When considering solution optimality as measured by the depth of
 generated circuit, one observation is that methods based on numerical
 optimization do not consider ancilla qubits. Another area of
 improvement is development of such methods. In our opinion, the
 easiest way is combining decomposition methods (Cosine-Sine) which
 already can handle ancillas with numerical optimization. 
  
  \parah{Synthesis for late NISQ (large) circuits} For circuits with
  tens of qubits memory and computational requirements for synthesis
  are prohibitive, as unitaries scale exponentially with $2^q$. Given
  an already existing circuit, a straightforward way to incorporate
  synthesis is to partition it in manageable size blocks, optimize
  these individually and recombine. For algorithm discovery, synthesis
  will have to be incorporated into generative models for domain
  science. For example, frameworks such as OpenFermion can already
  generate arbitrary size circuits. 
  
  
  




==> paper/impl.tex <==
\subsection{Implementation}
\label{sec:impl}

The pseudocode describing the algorithm  is presented in Figure{~\ref{fig:alg} and its behavior has been explained through the simple three qubit example in Figure~\ref{fig:usearch}.
  In the rest of this section we provide the implementation details which ultimately determine its performance and quality of solution.

\newcommand{\basetriangle}{% equilateral triangle with side 1
  \def\h{0.866025}% sqrt(3)/2
  \coordinate (X) at (-1/2,{-1/3*\h});
  \coordinate (Y) at (1/2,{-1/3*\h});
  \coordinate (Z) at (0,{2/3*\h});
  \fill[white!10, draw=black] (X) -- (Y) -- (Z) -- cycle;
  \filldraw (X) circle (3pt); \filldraw (Y) circle (3pt); \filldraw (Z) circle (3pt);
  }
  
\subsubsection{Customizing for QPU Gate Set and Topology}
  
  We target directly the gate set native to the quantum processor. Our initial implementation was tailored for the QNL8QR-v5 processor which supports in hardware the  {$R_x(90), R_z{\theta}, CNOT$} gates and its qubits are connected in a line topology. We have also re-targeted the algorithm for the IBM Q 5 qubit chip, with a similar native gate set but a bow-tie/triangle \begin{tikzpicture}[scale=0.5]
    \basetriangle
    
  \end{tikzpicture} topology. 


  
 While in the informal description of the algorithm we mention using a generic SU(2) unitary matrix $U3(\theta,\phi,\lambda)$, in the implementation we use the decomposition
\begin{equation}
  U3(\theta,\phi,\lambda) = R_z(\theta)R_x(90)R_z(\phi)R_x(90)R_z(\lambda)
\end{equation}


\red{Why is this decomposition correct? Cite where or prove...}


This decomposition still has three free parameters
$(\theta,\phi,\lambda)$ that need to be synthesized, but as $Z$
rotation gates have no hardware equivalent, it will generate only two
actual $R_x(90)$ hardware gates. On both processors $Z$ rotations are performed in software and accounted for at measurement time. Based on this decomposition, our synthesis will generate a number of $X$ rotations that is roughly twice the number of \cn gates.

Topology specialization is attained inside the {\tt get\_successors()} call in Figure~\ref{fig:alg} using a data structure that describes the qubit adjacency \red{\bf list/matrix}.

\subsubsection{Distance}

We use the following distance function based on the Hilbert-Schmidt inner product.
\begin{equation}
 D(U_{start},U_{goal}) = 1 -  \frac{\langle U, U_s \rangle_{HS}}{N} = 1 -   \frac{\Trace(U^{\dag} U_s)}{N}, where\ N\ is\ the\ number\ of\ qubits
\end{equation}


The formula is based on the fact that  the inverse of a unitary matrix is its conjugate transpose. If the synthesis succeeds and $U_{goal}$ is not distinguishable from U, the product $U_{goal}^{\dag}U = I_N$, where $I$ is the identity matrix.
Furthermore, the maximum magnitude that the trace of a unitary matrix can have is its size N, which occurs at the identity (up to a phase).
The closer $U^{\dag} U_s$ is to identity, the closer  $\frac{\Trace(U^{\dag} U_s)}{N}$ is to $N$, thus the closer our distance function is to $0$.

Note that variations of formulas using  Hilbert-Schmidt inner product have been previously used in synthesis algorithms~\cite{qaqc,ionsynth}, and ours has the following properties
\begin{itemize}
\item The distance is 0 when compilation is exact.
\item  It is easy to compute.
\item It has operational meaning.
\end{itemize}



%\lstinputlisting[language=Python,basicstyle=\tiny,numbers=right,emph={func}]{../pseudocodev2.txt}



==> paper/introduction.tex <==
\section{Introduction}
\label{sec:intro}

There is a high probability that quantum computing will deliver
transformational scientific results within the next few decades. Right
now, we are in an era of effervescence, where the first available~\citep{IBM-2017,Google-2018,Intel-2018}
hardware implementations of quantum processors have opened the doors
for exploration in quantum hardware, software and algorithmic
design. At the hardware level, chip designers keep introducing new
primitives  motivated by the desire  to model physical phenomena,
such as qutrits~\citep{qtrit,bhscramble} used 
to model information scrambling
in black holes. As current generation chips have relatively short
decoherence times, compile time  optimization of quantum circuits for depth
reduction is paramount to success in the near future. At the
algorithmic level, there exists a dire need for discovery combined
with a need for tools to assist in mapping a science level 
Hamiltonian to the equivalent circuit.

All three lines of exploration have in common that obtaining the
unitary matrix associated with the transformation (algorithm, gate,
circuit etc.) is ``easy'', while deriving equivalent circuits from said
unitary is hard.  Quantum circuit synthesis is an approach to derive a good circuit
that implements a given unitary and  can thus facilitate advances
in all these directions: hardware, software and  algorithmic exploration. 

Research into quantum circuit synthesis has a long history. The topic
was introduced by Solovay and
Kitaev~\citep{DawsonNielson05,Nagy16,ola15} which describe
the first algorithm to decompose an unitary into a circuit while
relating circuit depth to error.  The field has advanced a long way
since~\citep{ZXZ16,MIM13,Qcompile16,kmm13,GS13} in terms of synthesis quality and
runtime speed. For example,  for our native gate set target, our
Solovay-Kitaev implementation generates circuits of average 10,000 gates depth
for a sampling of random single qubit unitaries. In contrast, our
heuristic based algorithm generates circuits with at most \red{\bf five?} gates,
while performing
orders of magnitude faster.

We believe that synthesis can be a tool of great utility in the
quantum development kit for the Noisy Intermediate-Scale Quantum
Devices era, which is characterized by design space exploration at
small qubit scale. To foster acceptance and adoption,  implementations
need to become first  available for the existing generation of quantum
processors, while overcoming some of the currently perceived
shortcomings:
\begin{itemize}
\item Synthesized circuits tend to be deep.
\item Synthesis approaches handle poorly   the existing
  restrictive chip topologies.
\item The compilation itself is slow. 
\end{itemize}

In this paper we describe a  pragmatic heuristic synthesis
algorithm. We concentrate on
minimizing circuit depth while taking topology into account
 and {\it showing  usability in different scenarios: algorithm compilation,
 gate discovery and circuit optimization.} We demonstrate results
for
circuits with a small number of qubits, with the overall goal
of minimizing the number of \cn gates used in the resulting
circuit. As \cn has low fidelity on existing hardware and it is
expected to be the limiting factor in the near future of Noisy
Intermediate-Scale Quantum devices, this metric has been targeted by
others~\citep{raban,qaqc,synthcsd}. 

The algorithm is based on the A*~\citep{astar} strategy and works as
follows. Given the unitary associated with a quantum transformation,
we attempt to alternate layers of single qubit gates and \cn
gates. For each layer of single qubit gates we assign the generic
parameterized unitary to all the qubits. We then try to place a \cn
gate wherever the chip connectivity allows and pass the parameterized
circuit into an optimizer~\citep{cmaes}, in our case based on the Covariance Matrix
Adaptation Evolution Strategy (CMA-ES). Note that this approach allows
us to specialize for any given architecture with different qubit
connectivity. The optimizer instantiates the parameters
for the partial solution according to a distance
function. We now have a concrete, ready to compile circuit. At each step of the search, the solution closest to the
original unitary is expanded and the algorithm stops when the current
solution is within a small threshold distance from original. While
synthesis of quantum circuits using numerical optimization strategies
has been explored before~\citep{ionsynth,qaqc}, to our knowledge ours
is the first demonstration of a feasible manner of accounting for
chip connectivity. 

We initially  targeted the \qnl chip developed by the UC Berkeley
Quantum Nanoelectronics Laboratory ~\citep{qnl}, with eight
superconducting qubits connected in a line topology and with a native
gate set consisting of rotations and \cn gates \{$R_x(90),
  R_z(\theta), CNOT$\}.  We
demonstrate the efficacy of our approach for small circuits up to four qubits, in several usage
scenarios. The benchmarks consist of randomly generated single and
two-qubit unitaries and well known algorithms and gates published in
literature, e.g. QFT, HHL, Fredkin, Toffoli etc.

When compiling from
unitaries  to circuits, which is often the process
involved in algorithm discovery, in all cases we obtain
circuits with a \cn count considerably lower than  the tight upper bounds
provided by~\citet{raban}.  When comparing against numerical
optimization based techniques~\citep{ionsynth,qaqc}, again we seem to
generate similar or 
shorter circuits. For the \qnl chip, when comparing our
solution with the best implementation of a circuit/algorithm
published in literature we sometimes generate longer circuits. Whenever
this occurs, the difference is accounted by the \qnl chip connectivity
(or lack thereof).  When specializing the algorithm for a different
topology with better connectivity, such as the ``bowtie'' employed in
the IBM Q 5~\citep{ibmq5},
our algorithm can match the best known circuit depth\footnote{For
  convenience, we sometimes use ``depth'' to denote \cn gates count.}. For
example, for Fredkin gates on \qnl we generate circuits with nine \cn
gates, while on the IBM Q we use  eight \cn
gates, matching the best published implementation. \comment{\red{TBD - what happens if I compile the 6 gate Toffoli on a
  line? Maybe rigetti?}}

Our next usage case is demonstrating the use of synthesis in hardware
design space
exploration and gate discovery. First we show how our approach when starting
from unitaries can generate
circuits that implement   qutrit
gates~\cite{qtrit}. In this case we match the depth of hand generated
and optimized circuits. Perhaps more interesting for the short term,
is the exploration of $\sqrt{\cn}$ gates. More than once, in our
discussions with hardware designers the topic  of their usability
came up, and they are actively considered in industry and academia as
an alternative to \cn.  When using our synthesis algorithm, results show that in all
cases considered, circuits using only  $\sqrt{\cn}$ instead of \cn have identical or shorter length, therefore likelier to
have  higher fidelity. This demonstrates the extensibility of our
approach and  shows
empirical evidence that synthesis can be used to co-design the
processor gate set together with the compilation toolchain. 

The last usage case is demonstrating the efficacy of synthesis in
  circuit optimization.  In this case we start with known circuits,
  lift them to unitaries and re-synthesize. In all cases, we obtain
  circuits of equal or smaller length.

Overall, we believe that we have made several good contributions that
advance the state of the art in quantum circuit synthesis. We have
shown how to synthesize short circuits while using chip
topology information, and we provide quantitative data for a
reasonably large suite of benchmarks. In contrast, some state-of-the-art
synthesis approaches~\citep{raban,synthcsd}  prove only bounds on circuit depth, without
quantitative data on specific circuits. Furthermore, they report large
proportionality   constants that affect the circuit depth when
specializing for topology. Our practical results demonstrate a much
lower overhead. Our algorithm seems to be flexible, allows for gate
set re-targeting and design space exploration, in contrast with
previous approaches that only 
consider fixed gate sets. When comparing with other empirical techniques based on
numerical optimization and search~\citep{ionsynth,qaqc}, we generate
shorter circuits, can handle topology and provide a more extensible approach.  This provides tangible proof
that synthesis can be useful for quantum algorithm and systems
co-design at the small NISQ device qubit count, and supplements most existing synthesis studies with a wide
suite of quantitative results. 
Furthermore, since most quantum
processors using 
superconducting qubits support very similar gate sets and the
algorithm takes qubit interconnection into account, we believe the our
approach is generic and easily extensible to  other chip
architectures, native gate sets and topologies.

The rest of this paper is structured as follows. In
Section~\ref{sec:bg} we introduce the problem, its motivation and
provide a short primer on quantum computing. In
Section~\ref{sec:alg} we describe our algorithm and its
implementation, while in Section~\ref{sec:use} we present results for
the three usage scenarios. In Section~\ref{sec:prop} we analyze the
algorithm behavior. In Section~\ref{sec:related} we describe the related work,
while in Section~\ref{sec:disc} we discuss future uses of synthesis in
the NISQ era. 

==> paper/misc.tex <==
\subsection{To Do}

\begin{enumerate}
\item Mention Shende synthesis paper - topology adds a factor of nine in CNOTs ...


\item Raban and Shende - algorithms only, upper bounds with no implementation


\item Sutton - not that many real algorithms to compute CSD

\item CSD may not apply to qutrits ...

\item ~\citep{MIM13} Clifford+T - they do Toffoli, 10 CNOTS + 2 Ts, don't scale...

\item\citep{ionsynth} - needs discussion. Numerical optimization with
  predecomposed matrix with MS gates (equivalent to CNOTs). 3 qubits
  in 8 gates - we do better. Not topology aware, does not matter for
  MS. Decomposition fixed for qubits and CNOTs - can't specialize
  easily. Search strategy - random seed and search ..

  \item \citep{qaqc} - same idea for numerical optimization, but use
    quantum computer for it. Show results for 2 qubits, which we
    match. Simulated annealing over all sequences of length L. Same
    metric based on Hilbert-Schmidt.
  
\item Discussion section - what is synthesis good for. We show its a
  good tool for small circuits, probably gate discovery, circuit
  optimization with partitioning...
  Discuss scalability trends and possible approaches: partitioning,
  norm selection ...

\end{enumerate}

==> paper/related.tex <==
\section{Related Work}
\label{sec:related}

A fundamental result in the theory of quantum computation, which
spurred the apparition of quantum circuit synthesis is provided by the
Solovay Kitaev (SK) theorem. This states that, intuitively, it is possible
to obtain good approximations to any desired gate ($(SU(2)$) using surprisingly
short sequences of gates from a given generating\footnote{With
  constraints on this set to be dense in SU(2).} set. The theorem
relates circuit depth to the quality of the approximation and its
proof is by construction ~\citep{DawsonNielson05,Nagy16,ola15}.

In practice,
``surprisingly short'' in mathematical terms turned unacceptable to run on
physical devices, and different approaches~\citep{DawsonNielson05,ZXZ16,BocharovPRL12,MIM13,Qcompile16,ctmq,23gates,householderQ,CSD04,amy16,seroussi80} to synthesis have been
introduced since, with the goal of generating shorter depth circuits. 

The existing approaches can be coarsely classified based on several
criteria: 1) target gate set; 2) the distinguishability of the
solution; and 3) their
algorithmic approach.


\parah{Target Gate Set} The SK algorithm is quite general in the sense that it is applicable to any 
universal gate set. Synthesis can be improved in terms of both speed
and  optimality by specializing the gate set.  For example, the z-rotation unitaries can be
synthesized with Clifford+V approximation~\cite{Ross15} or  with Clifford+T gates~\cite{KMM16}. The set of Pauli, Hadamard, Phase, CNOT 
gates form what is known as the Clifford group gates. When augmented with the T gate defined
as 
\[
T = \left(
\begin{array}{cc}
1 & 0 \\
0 & \zeta_8 
\end{array}
\right), \ \ \mbox{where} \ \ \zeta_8 = e^{i\pi/4},
\]
the gate set is universal. When ancillary qubits are allowed, one can synthesize
a single qubit with the Clifford+T gate set~\cite{KMM16,KSV02,Paetznick2014}. 
It lead to better complexity $\mathcal{O}(\log^{1.75}(1/\epsilon))$ compared 
to the SK Algorithm.  \comment{$\mathcal{O}(\log(1/\epsilon))$ T-count scaling.}

While these efforts propelled the field of synthesis, they are not 
used on NISQ devices, which offer a different gate set
($R_x, R_z,CNOT$ and M\o lmer-S\o rensen all-to-all).
Several~\citep{raban,synthcsd,ionsynth}  other
algorithms, discussed below have since emerged.

\parah{Solution Distinguishability} 
Synthesis algorithms are classified as exact or approximate based on
distinguishability.  This is a subtle classification criteria, as most
algorithms can be viewed as either.  For example,~\citet{MIM13} proposed a divide-and-conquer algorithm called Meet-in-the-Middle (MIM).
It allows one to search for
circuits of depth $l$ by only generating circuits of depth at most $\lceil l/2 \rceil$ at the complexity of $\mathcal{O}(|\mathcal{V}_{n,\mathcal{G}}|^{\lceil l/2\rceil}\log |\mathcal{V}_{n,\mathcal{G}}|^{\lceil l/2 \rceil})$, 
where $\mathcal{V}_{n,\mathcal{G}}$ denotes the set of unitaries for depth-one 
$n$-qubit circuit. The MIM algorithm is flexible and allows weights to be
added to the gate set to account for the possibility that some gates,
such as those that do not belong to the Clifford group, may be more expensive
to implement. It also allows ancillas to be used in the synthesis.  The 
algorithm uses a number of heuristics to prune the search tree.  Although
it was originally designed for exact circuit synthesis, the algorithm
may also be used to construct an $\epsilon$-approximate circuit.

Furthermore, on NISQ devices, the target gate set of the algorithm
(e.g. T gate) may
be itself implemented as an approximation when using native gates.

We classify our approach as approximate, in the sense that to improve
the speed we accept solutions at a small distance from the original
unitary. We could also impose a zero distance if exact synthesis is
necessary. 


\parah{Algorithmic Approaches} The earlier attempts inspired by
Solovay Kitaev use a recursive (or divide-an-conquer) 
formulation, sometimes supplemented with search heuristics at the
bottom. More recent search based approaches are illustrated by the
Meet-in-the-Middle algorithm.


Several  approaches use techniques from linear algebra for
unitary/tensor decomposition.  \citet{23gates} use QR matrix factorization via Given's rotation and Householder transformation
~\citep{householderQ}, but there are open questions as to the suitability
for hardware implementation because these algorithms are expressed 
in terms of row and column updates of a matrix rather than in terms of qubits. 
\citet{CSD04} use Cosine-Sine
transformation,~\citet{BocharovPRL12} use KAK transform
and Clifford+T decomposition to reduce a unitary transformation on $w$-qubit to a cascade
of unitary transformation on $(w-1)$-qubits.

The state-of-the-art upper bounds on circuit depth are provided by
techniques~\citep{synthcsd,raban} that use Cosine-Sine
decomposition. The Cosine-Sine decomposition was first
used by~\citet{tucci}  for compilation purposes. 
Cosine-Sine decomposition states that every unitary matrix $ U \in
\mathbb{C}^{2^n \times 2^n}$ 
can be decomposed in terms
$A_0 , A_1 , B_0 , B_1 \in \mathbb{C}^{2^{(n-1)} \times 2^{(n-1)}}$ and
real diagonal matrices C and S, where  $C^2 +S^2 = I$

\begin{equation} \label{eq:rs}
U =  \begin{pmatrix} A_0  & 0 \\  0& A_1\end{pmatrix} \begin{pmatrix}
  C & -S \\   S & C\end{pmatrix}\begin{pmatrix} B_0  & 0\\   0 &  B_1\end{pmatrix}
\end{equation}

The basic formulation of these techniques is topology
independent. Specializing for topology increases the upper bound by
rather large constants (~\citet{synthcsd} mention a factor of nine)
for the NISQ devices purposes. As discussed, the question remains whether other empirical
techniques~\citep{ionsynth,qaqc}, including ours, can generate even
shorter circuits.  The published approaches targeting qubit based
systems cannot
handle new primitives such as qutrit gates and work for generalization
is required. Furthermore, it seems that the numerical
techniques~\citep{computecsd} required for CSD still require
refinements as they cannot handle numerically challenging cases.

There are not many studies published about synthesis of qutrit based
circuits and qutrit gate sets.~\citet{qtsynth} describes a method
using Givens rotations and Householder decomposition. As techniques
for qubit based systems using a similar approach have been
proposed~\citep{23gates}, they may allow an easier combination of
qutrit and qubit based synthesis. 

Several techniques use numerical optimization, much as we did. They
describe the gates in their variational/continuous representation and
use optimizers and search to find a gate decomposition and
instantiation.
The work closest to ours is by~\citet{ionsynth} which  use
numerical optimization and brute force search to synthesize circuits
for a processor using trapped ion qubits. Their main advantage is the
existence of all-to-all M\o lmer-S\o rensen gates, which allow a topology
independent approach. When Martinez et al. describe their results,
they claim that M\o lmer-S\o rensen counts are directly comparable to CNOT
counts. By this metric, we seem to generate comparable or shorter
circuits than theirs.  It is not clear how their approach behaves when
topology constraints are present. The direct comparison is further limited due to
the fact that they consider only randomly generated unitaries, rather
than algorithms or well understood gates such as Toffoli or Fredkin.

Another topology independent numerical optimization technique is
presented by~\citet{qaqc}. In this case, the main contribution is to
use a quantum annealer to do searches over sequences of increasing
gate depth. They report results only for two qubit circuits.

All existing studies focus on the quality of the solution, rather than
synthesis speed. They also report results for low qubit concurrency:
Khatri et al. for two qubit systems, Martinez et al. for systems up to
four qubits.










==> paper/setup.tex <==
\section{Experimental Setup} 
\label{sec:exp}


\parah{Software Implementation}  The code is implemented in Python 3.0 using {\tt numpy}. The optimizer is the CMA-ES PyPI~\citep{cmaes,cmapy} implementation.  Most of the tests ran on a 2017 MacBook Pro laptop, the four qubit tests ran on 16 core server grade processors  Intel Xeon  E5-2698 v3 ("Haswell") at 2.3 GHz.

The algorithm step to expand the next solution is parallelized using the {\tt multiprocessing} Python package and the {\tt imap\_unordered} process pool policy which allows for asynchronous evaluation of partial solutions.

We were initially most interested in the quality of the synthesis solution, rather than execution speed. As results indicate that the numerical optimizer seems to be the performance bottleneck, further optimization of the parallelization strategy may not be warranted.

\red{\bf NEED statement about stopping criteria, error threshold.}






==> paper/use.tex <==


\section{Use Cases}
\label{sec:use}

\newcommand{\linett}{% side 1
 
  \coordinate (Y) at (0,0);
  \coordinate (Z) at (0,1);
  \fill[white!10, draw=black] (Y) -- (Z);
 \filldraw (Y) circle (3pt); \filldraw (Z) circle (3pt);
}

We concentrate on algorithms spanning a small number of qubits as we are interested in compiling for the Noisy Intermediate-Scale Quantum devices. Our goal is to demonstrate the value of synthesis to practitioners under several usage scenarios: 1) algorithm discovery; 2) gate set design exploration;  and 3) circuit optimization.

To showcase algorithm discovery we select ``traditional'' algorithms or quantum transformations, when using the native single and two-qubit gates on the two quantum processors described in Section~\ref{sec:qps}. Table~\ref{tab:res} presents a summary of our results. We use randomly generated unitaries,  logical gates (Toffoli, Fredkin, Peres) and the unitaries associated with known algorithms such as Grover search~\citep{grover}, Quantum Fourier Transform~\citep{qft} and HHL~\citep{hhl}.

As the native gate sets are similar, the distinguishing characteristic is the qubit interconnection topology, provided in the column headings.  For the current generation hardware, the reader should focus on the columns where we target directly the \cn gates.

To showcase gate set design exploration we consider two scenarios: 1) replacing \cn gates with $\sqrt{\cn}$ gates, a problem of current interest to both (UCB and IBM) hardware design teams; and 2) synthesis of qutrit gates, a problem of interest to hardware (UCB)  and algorithm designers.

Finally, we consider using  synthesis during the circuit optimization phase. 




\subsection{Synthesis for Algorithmic Discovery - Compiling Unitaries to Circuits}

This is the use case explored most by the existing body of work in quantum circuit synthesis. The premise here is that it is easier for domain scientists to obtain an unitary matrix associated with their algorithm, than to derive the circuit directly. This happens in physical sciences, as well as during gate design, where logical gates need to be instantiated into hardware native gates.

In all cases illustrated in Table~\ref{tab:res} we were able to synthesize circuits shorter than the theoretical upper bounds provided by ~\citet{raban}.  Their \cn count upper bounds for Q=2 and Q=3 are 3 and 20 respectively.

When examining the results for the line topology (\begin{tikzpicture}[scale=0.3]
    \linett
  \end{tikzpicture}), sometimes we match the shortest circuit depth
  available in literature, sometimes we exceed it.  Note that the
  shortest circuit depth published has been obtained after thorough
  manual optimization. On the line topology, whenever we exceed the optimal known depth for
  a circuit, the results are attributed to lack of
  connectivity.  These circuits cannot be implemented on a line
  topology at their published depth. 

  For two qubit circuits we always match the shortest depth
  available. For the three qubit Toffoli  gate, HHL and QFT  we match or exceed (QFT) the best
  published depth. The Fredkin gate  on a line topology is usually
  implemented using three Toffoli gates, which accounts for a depth of
  27 \cn gates. The end Toffoli gates can in theory be replaced by
  CNOT gates, but this transformation requires full connectivity to
  work. 

  For Toffoli and Fredkin gates, circuits with shorter CNOT count are
  available in literature. Matching this requires topology
  specialization.  We present results for the IBM bowtie/triangle and
  this is where things get interesting. In most cases we match or
  provide lower depth than in the line topology. For QFT we reduce
  depth from eight to seven.

 The best known depth for Toffoli is a  circuit with six \cn gates. In our experiments we obtain nine
 gates. In this case, the search has found a solution that satisfies
 our stopping criteria. 

 \comment{Similarly,~\citet{noisemap} use a Fredkin implementation that
  is eight deep, while we obtain a depth of nine. These two cases
  expose a very subtle limitation of all numerical optimization based synthesis
  techniques currently published.

  As described in Section~\ref{sec:related}, modulo the expansion
  strategy, all  numerical optimization techniques alternate layers of CNOT and arbitrary
  single qubit gates in an attempt to reduce the dimensions of the
  search space. On the other hand, when examining the optimal
  implementations of Toffoli and Fredkin, the circuits contain a
  number of single qubit gates  lower than in any circuit synthesized by
  numerical optimization approaches. For Fredkin, the implementation used
  in~\citep{noisemap} uses 11 single qubit gates, while our algorithm
  will insert $3+8 \times 2 = 19$ gates. A similar situation occurs
  for Toffoli. In the ideal case, one would expect the numerical
  optimizer to be able to synthesize identity gates wherever
  necessary, but this does not seem to be the case. We are working to
  empirically validate this conjecture. If true, this insight
  indicates that synthesis can be improved by either more informed
  expansion strategies or by customized numerical optimization algorithms.}
 

 \subsection{Synthesis and Gate Discovery - $\sqrt{\cn}$ and Qutrits} 



\begin{figure}
  \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
    ALG & Q   & CNOT  \begin{tikzpicture}[scale=0.4]
    \linett
    \end{tikzpicture}  & $\sqrt{CNOT}$\begin{tikzpicture}[scale=0.4]
    \linett
    \end{tikzpicture} & CNOT \begin{tikzpicture}[scale=0.5]
    \basetriangle
    
  \end{tikzpicture} &  $\sqrt{CNOT}$ \begin{tikzpicture}[scale=0.5]
    \basetriangle
    
  \end{tikzpicture} \\
    \hline
    \hline
    SU(2) &
2&
3&
   3& &  \\
    \hline
QFT &
2 &
3&
   3& 3& 3 \\
    \hline
    \hline
   
Toffoli & 3 & 9 & 9 & 9 & 10 \\
    \hline
 Peres&
3&
9&
   9&
      9&
            \\
    \hline
Fredkin & 3 &>20*& 9  & 8 &  \\
    \hline
    \hline
HHL &3 &4&4 &\red{5} &  \\
    \hline
QFT &3&8&8&7& 8 \\
 %   \hline
  % Grover &
%3 & ??&
 %     ??  & ?? & ?? \\
    \hline 
  \hline
  VQE 
ethylene &
4 &
    >27* &  &  &  \\
    \hline
  \end{tabular}
  \caption{\label{tab:res}\it  Summary of synthesis results for
    several algorithms and unitaries. Q = number of qubits. The
    topology used during synthesis is denoted in the
    caption. Theoretical \cn count upper bounds for Q=2 and Q=3 are 3
    and 20 respectively. Numbers with * denote runs that took to long
    to finish on a laptop. These were expected to fail due to
    limitations in the numerical optimizer. The Fredkin gate can be
    implemented using three Toffoli gates, with a depth of at least 27
  \cn gates on a line topology. The original VQE circuit has a depth
  of 64 \cn gates. }
\end{figure}



\subsubsection{$\sqrt{\cn}$ Gates}
Two {$\sqrt{\cn}$ gates applied in sequence to a pair of
  qubits  are not distinguishable from CNOT gate.  
These  gates often come up in conversations with hardware
designers. One line of reasoning is that they may be easier to
calibrate than  a proper CNOT.

Recent yet unpublished work at the IBM
QISKit 2019 boot-camp showed shorter circuits when using a combination
of $\cn$ and $\sqrt{\cn}$ gates. To our knowledge, IBM is seriously considering
adding a native $\sqrt{\cn}$ gate to their IBM Q architecture. This will be mutually exclusive with the proper
\cn gate.

From our perspective, as long as CNOT gates are mutually exclusive,
the more important reason is that $\sqrt{\cn}$ is a building block to
the universal gate CRZ  described in Figure~\ref{fig:crz}. A
legitimate question is whether circuits can be shorter when using
CRZ as the only two qubit gate. When starting this line of exploration, we have
constructed example unitaries that are clearly implemented with
shorter circuits when using CRZ gates, results omitted for brevity.
The question remains whether the same occurs in any existing
circuit or gate unitaries.



In our algorithm, we replace CNOT with CRZ in the basic expansion
block described in Figure~\ref{fig:usearch} (A).   Note that this adds
one extra parameter at each expansion step, increasing from six to
seven. The results in
Table~\ref{tab:res} indicate  that in most cases we can synthesize
circuits at the same depth with CNOT or CRZ. One notable exception is
the Fredkin gate, which on a line topology can be implemented using
three Toffoli gates, with a depth of 27 CNOT gates. With CRZ, the
resulting depth is only nine.

We believe this demonstrates the value
of considering CRZ and implicitly $\sqrt{\cn}$ gates as basic building
  blocks. Note that this alternative, to our knowledge, has not been
  previously considered. 
  

\begin{figure}
    \includegraphics[width=2in,height=1in,keepaspectratio]{crz}
    \caption{\label{fig:crz} \it CRZ universal gate, its unitary introduces seven
      unbounded parameters.}
\end{figure}





\subsubsection{Qutrits}

Qutrits extend qubits to systems with three logical values 0, 1 and
2. They are represented by unitaries from SU(3) and extend from binary
to ternary logic to 
explore a space with $3^n$ dimensions. There exist several~\citep{qtsynth,qtparam}
decompositions and parameterizations, all using eight independent
parameters. Gates to implement qutrit operations  have been explored only
recently~\citep{qtrit} for qubit based systems, mostly motivated by
the need~\citep{bhscramble}  for
modeling  physical phenomena. 

For our study, we implement a CSUM two-qutrit gate, which adds the
value of the first qutrit to the second qutrit $CSUM(\ket{11}) = \ket{12}$.  Our synthesis matches
the hand optimized implementation  by~\citet{qtrit}. For ASPLOS submission
time brevity we
omit the qutrit parameterization, the CSUM unitary and the structure of
the synthesized circuit. 

To our knowledge, this is the first practical demonstration of qutrit
gate synthesis on qubit based systems. 


\subsection{Synthesis and Circuit Optimization}

The last use case we consider is incorporating synthesis in quantum
compilers for circuit optimization purposes.  To our knowledge, this
is the only technique able to reduce CNOT count/depth in non trivial
cases and it is currently not deployed. Existing compilers for quantum
programming languages tend to use simple peephole optimizations and
circuit rewriting techniques.

One common practice for developers is  to take existing published
implementations of algorithms and port them to the target quantum
processor. Often the circuits are described in terms of logical rather
than native gates. When run through existing compilers or optimized by
hand, the resulting circuit is often suboptimal. This is illustrated
by Figure~\ref{fig:hhl} where we examine a hand optimized
implementation of HHL obtained from the QNL8QR-v5 development
team. Their circuit contains seven \cn gates, while our solution
contains only four. 

\begin{figure}
    \includegraphics[width=3in,height=1.5in,keepaspectratio]{hhl}
    \caption{\label{fig:hhl} \it  HHL hand optimized circuit compared
      to synthesized solution. }
\end{figure}

When considering two and three qubit circuits (or partitions of a
larger circuit) our results indicate that synthesis can be a useful
tool.  For example,~\citet{noisemap} report using a QFT two qubit
implementation with five \cn gates. Our synthesis package was able to
regenerate a circuit with three \cn gates.

The need for aggressive optimizations is further motivated by the emergence of
circuit generators. At the application or domain science layer, packages such as
OpenFermion~\citep{openfermion} produce circuits by translating from
physics or chemistry  first
principles. Due to the complexity of the
problem, the generated circuits are often long and suboptimal. At the
compiler level, it is worth exploring approaches for ``global''
circuit optimization, where circuits (or partitions thereof) are
lifted to unitaries and re-synthesized.



In Table~\ref{tab:res} the entry labeled ``VQE ethylene'' corresponds
to a four qubit circuit generated by OpenFermion to simulate  the ethylene
molecule. The circuit contains 64 \cn gates. We
lifted the circuit to the unitary matrix and attempted to
re-synthesize it. As illustrated, we have aborted the compilation at a
depth of 27 due to its long duration. As the bottleneck is the
numerical optimizer performance at large parameter count, circuit
partitioning techniques are needed when increasing the qubit count. 









